MEL: Coordinate-Preserving EEG Tokenization for fMRI Translation

Background and Objective: Predicting regional blood-oxygen-level-dependent (BOLD) activity from EEG provides a computational approach to studying electrophysiological-hemodynamic associations. However, changes in input representation, readout architecture, and ensembling can obscure the source of a prediction gain. We investigate the contribution of target-relative spectral estimation under matched readout conditions. Methods: MEL converts each preceding 16-second EEG history into calibrated lag-channel-frequency measurements. Four equal-dimensional representations are compared using matched Ridge and multilayer perceptron (MLP) readouts. The retrospective analysis includes 29 resting-state scans from 22 participants, participant-paired uncertainty estimates, aggregation and correspondence controls, leave-one-participant-out regression, and refitted models on an external Oddball cohort. Results: Morlet-Ridge achieved a mean scan-wise correlation of 0.508 across six regional targets and the global signal, compared with 0.432 for canonical Fourier features. The participant-paired mean difference was 0.069 (95% bootstrap confidence interval, 0.037-0.101), with improvements in 19 of 22 participants. The Morlet MLP prediction ensemble reached 0.491. Shared coordinate permutations preserved prediction after refitting, whereas sample-wise permutations degraded it. Canonical Fourier regression reached 0.377 under participant exclusion; external unseen-participant correlation was 0.026. Conclusions: Spectral estimation materially affected regional BOLD prediction without requiring additional nonlinear readout capacity. MEL provides an explicit measurement interface for controlled comparisons, but weak external results constrain its generalizability. Confirmation requires untouched participant-separated data and split-aware preprocessing.

==> references.tex <==
\begin{thebibliography}{99}
\bibitem{huster2012}
R.J. Huster, S. Debener, T. Eichele, C.S. Herrmann,
Methods for simultaneous EEG--fMRI: an introductory review,
J. Neurosci. 32 (2012) 6053--6060.
\url{https://doi.org/10.1523/JNEUROSCI.0447-12.2012}.
\bibitem{abreu2018}
R. Abreu, A. Leal, P. Figueiredo,
EEG-informed fMRI: a review of data analysis methods,
Front. Hum. Neurosci. 12 (2018) 29.
\url{https://doi.org/10.3389/fnhum.2018.00029}.
\bibitem{logothetis2001}
N.K. Logothetis, J. Pauls, M. Augath, T. Trinath, A. Oeltermann,
Neurophysiological investigation of the basis of the fMRI signal,
Nature 412 (2001) 150--157.
\url{https://doi.org/10.1038/35084005}.
\bibitem{buxton1998}
R.B. Buxton, E.C. Wong, L.R. Frank,
Dynamics of blood flow and oxygenation changes during brain activation: the balloon model,
Magn. Reson. Med. 39 (1998) 855--864.
\url{https://doi.org/10.1002/mrm.1910390602}.
\bibitem{mantini2007}
D. Mantini, M.G. Perrucci, C. Del Gratta, G.L. Romani, M. Corbetta,
Electrophysiological signatures of resting state networks in the human brain,
Proc. Natl. Acad. Sci. USA 104 (2007) 13170--13175.
\url{https://doi.org/10.1073/pnas.0700668104}.
\bibitem{scheeringa2011}
R. Scheeringa, P. Fries, K.M. Petersson, R. Oostenveld, I. Grothe,
D.G. Norris, P. Hagoort, M.C.M. Bastiaansen,
Neuronal dynamics underlying high- and low-frequency EEG oscillations contribute independently to the human BOLD signal,
Neuron 69 (2011) 572--583.
\url{https://doi.org/10.1016/j.neuron.2010.11.044}.
\bibitem{calhas2023}
D. Calhas, R. Henriques,
EEG to fMRI synthesis benefits from attentional graphs of electrode relationships,
Proc. Mach. Learn. Res. 219 (2023) 76--93.
\url{https://proceedings.mlr.press/v219/calhas23a.html}.
\bibitem{li2024}
Y. Li, A. Lou, Z. Xu, S. Zhang, S. Wang, D.J. Englot, S. Kolouri,
D. Moyer, R.G. Bayrak, C. Chang,
NeuroBOLT: resting-state EEG-to-fMRI synthesis with multi-dimensional feature mapping,
Adv. Neural Inf. Process. Syst. 37 (2024).
\url{https://doi.org/10.52202/079017-0736}.
\bibitem{lanzino2024}
R. Lanzino, F. Fontana, L. Cinque, F. Scarcello, A. Maki,
NT-ViT: neural transcoding vision transformers for EEG-to-fMRI synthesis,
arXiv preprint (2024).
\url{https://doi.org/10.48550/arXiv.2409.11836}.
\bibitem{roos2025}
K.G. Roos, A. Fukuda, Q.H. Cap,
From brainwaves to brain scans: a robust neural network for EEG-to-fMRI synthesis,
arXiv preprint, version 3 (2025).
\url{https://doi.org/10.48550/arXiv.2502.08025}.
\bibitem{kim2026}
E. Kim, J.K. Gahm,
MARBLE: lightweight EEG-to-fMRI translation via Mamba-attention and ROI-conditioned decoding,
Medical Image Computing and Computer Assisted Intervention -- MICCAI 2026,
LNCS 16894, Springer Nature Switzerland (2026).
\url{https://papers.miccai.org/miccai-2026/0612-Paper4437.html}.
\bibitem{dadi2020}
K. Dadi, G. Varoquaux, A. Machlouzarides-Shalit, K.J. Gorgolewski,
D. Wassermann, B. Thirion, A. Mensch,
Fine-grain atlases of functional modes for fMRI analysis,
NeuroImage 221 (2020) 117126.
\url{https://doi.org/10.1016/j.neuroimage.2020.117126}.
\bibitem{walzdata}
J.M. Walz, R.I. Goldman, J. Muraskin, B.R. Conroy, T.R. Brown, P. Sajda,
Simultaneous EEG and fMRI during a three-stimulus oddball task,
OpenfMRI dataset ds000116.
\url{https://openfmri.org/dataset/ds000116/} (accessed 11 October 2026).
\bibitem{yang2023}
C. Yang, M.B. Westover, J. Sun,
BIOT: biosignal transformer for cross-data learning in the wild,
Adv. Neural Inf. Process. Syst. 36 (2023) 78240--78260.
\url{https://doi.org/10.52202/075280-3420}.
\bibitem{wang2025}
J. Wang, S. Zhao, Z. Luo, Y. Zhou, H. Jiang, S. Li, T. Li, G. Pan,
CBraMod: a criss-cross brain foundation model for EEG decoding,
International Conference on Learning Representations (2025).
\url{https://proceedings.iclr.cc/paper_files/paper/2025/hash/bbbd6d915cb90be21c1254a82d45cedd-Abstract-Conference.html}.
\bibitem{zhou2025}
Y. Zhou, J. Wu, Z. Ren, Z. Yao, W. Lu, K. Peng, Q. Zheng, C. Song,
W. Ouyang, C. Gou,
CSBrain: a cross-scale spatiotemporal brain foundation model for EEG decoding,
arXiv preprint (2025).
\url{https://doi.org/10.48550/arXiv.2506.23075}.
\end{thebibliography}

